Solving Rearrangement Puzzles using Path Defragmentation in Factored State Spaces

Rearrangement puzzles are variations of rearrangement problems in which the elements of a problem are potentially logically linked together. To efficiently solve such puzzles, we develop a motion planning approach based on a new state space that is logically factored, integrating the capabilities of the robot through factors of simultaneously manipulatable joints of an object. Based on this factored state space, we propose less-actions RRT (LA-RRT), a planner which optimizes for a low number of actions to solve a puzzle. At the core of our approach lies a new path defragmentation method, which rearranges and optimizes consecutive edges to minimize action cost. We solve six rearrangement scenarios with a Fetch robot, involving planar table puzzles and an escape room scenario. LA-RRT significantly outperforms the next best asymptotically-optimal planner by 4.01 to 6.58 times improvement in final action cost.

==> src/02_deprecated.tex <==

\section{Deprecated Related Work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
There are two common approaches to addressing rearrangement puzzles that concentrate on utilizing the full robot-object configuration space: symbolic- and constrained-based approach

In a \emph{symbolic planning} approach~\cite{toussaint2018RSS, Hartmann2021TRO, garrett2018ffrob}, we create a search graph over symbolic actions (e.g., pick, place), applicable to each of the objects in the scene. A valid path through this search graph provides an action skeleton, a set of constraints usable for motion planning~\cite{Grothe2022} or differentiable optimization~\cite{toussaint2015IJCAI}. If an action skeleton is infeasible, expensive backtracking has to be performed~\cite{20-driess-RSS} to validate another action skeleton. In scenes with multiple objects, which have to be moved out of the way to solve the problem, such approaches might spend considerable time re-validating action skeletons. 

Our work is complementary, in that we also execute symbolic actions on our robot, but we choose those actions \emph{implicitly} using the (admissible) heuristic from our \puzzlealgo planner, which gives us a complete valid sequential solution path for all objects involved. This tighter integration of planning and robot capabilities give us a better chance to avoid expensive backtracking.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Second, rearrangement puzzles can be solved using a \emph{constrained-based planning approach}~\cite{kingston2018sampling, Kingston2019, vega2020asymptotically, lozano2014constraint,garrett2018sampling,mirabel2017manipulation}. Instead of only relying on symbols, in this approach, we enumerate all constraints using a constraint graph, which provides information about the inter-connectivity of constraint sets. To find solutions, we can employ constrained-based sampling, where uniform sampling is combined with projection methods, which project samples down onto a desired constraint-set or used as steering method~\cite{berenson2011task, Kingston2019}. Such methods avoid the difficulty of finding good symbols for a particular problem, but they become sample-inefficient when the projection methods do not adequately cover all constraint-sets. 

Our approach differs in that we do not plan directly in the full robot-object configuration space, which can be costly to compute. Instead, we integrate the capabilities of the robot into the motion planner using the new factored state space (see Sec.~\ref{sec:problemstatement}) to ensure correct paths are returned.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Rearrangement puzzles can also be solved using existing asymptotically optimal planners such as RRT*~\cite{karaman2011sampling}, PRM*\cite{karaman2011sampling}, FMT*~\cite{janson2015fast} or BIT*~\cite{gammell2020batch} or with state-of-the-art optimal motion planners like ABIT*~\cite{strub2020abit} or AIT*~\cite{strub2021ait}. However, the solution path will not be manipulatable by a robot. More specifically, the solution would move all objects simultaneously and reach the solution, which is not possible to manipulate if we have only one robot arm. Therefore, a different state space is needed to distinguish between the objects. Our new factored state space allows us to differentiate between the objects in the state space and thus in the solution path, thereby making it possible to extract the found actions. However, this is not enough to find a low number of actions executable by a robot. Most planners deliver very high action cost results and can not fully exploit our factored state-space. Therefore, another optimization step is needed in order to reach the lowest number of actions to solve the problem, which we present in \ref{sec:pathdefragmentation}.


Solving rearrangement problems with a hierarchical planning approach in combination with multi-modal planning has also been proposed~\cite{barry2010hierarch,kaelbling2010hierarchical}. The idea is to divide the task and motion planning into two layers. The lower layer considers the planning of a path for an object, which is then used to determine the necessary transfer modes along that found path in the upper layer. Similarly, in our approach, we first solve the object-only problem using the factored state-space and then deliver the solution, i.e., the found action sequence, to the robot to manipulate the tasks. However, in our case of rearrangement puzzles, it is crucial not only to find a path for the objects but also finding the minimal number of actions. Most hierarchical approaches are investigated in uncluttered environments~\cite{barry2010hierarch,kaelbling2010hierarchical} and refer to Navigation Among Moving Obstacles (NAMO) ~\cite{stilman2008planning} problems for rearrangement problems where the order of the movement of the objects is crucial. 

We also share similarities to NAMO~\cite{stilman2008planning} problems that focuses on finding a path for the robot in an environment of movable obstacles whose goal poses are not predetermined while optimizing certain cost criteria, e.g., the number of displaced objects. On the other side, most of the investigated rearrangement planning problems only consider predetermined start and goal poses for each object~\cite{krontiris2015dealing,gao2021fast,gao2021minimizing}.  In our case, rearrangement puzzles, we generalize the idea of both types of these problems by proposing a new planner that is capable of handling both types of goals and demonstrate a way in which we can efficiently solve them.

Additionally, NAMO problems can be divided into \emph{monotone} and \emph{non-monotone} problems~\cite{stilman2008planning}. Monotone problems describe the problems where the objects in the problem can be manipulated only once, whereas in non-monotone problems the objects need to be manipulated multiple times. Our factored approach is capable of handling both kinds of problems. 

% maybe take this part out too? to win some space?

Our approach relies on finding optimal solutions to motion planning problems in our factored state space. This is closely related to planners like Manhattan-like RRT~\cite{Cortes2007}, where planning is decomposed into an active and a passive subspace. Planning is done exclusively in the active subspace, while the passive subspace is only sampled when obstructions are detected (for example, when a door blocks an object). Our planner generalizes this idea, makes it applicable to manipulation, and combines it with optimality, such that we find the minimal amount of switches between subspaces.\\


%Our approach aims to minimize the necessary number of actions to solve the problem. This is also explored in assembly sequence planning~\cite{masehian2020asppr} to find an action sequence with the minimum number of \emph{relocations} by focusing on the interferences between objects. Another approach~\cite{wang2021uniform} for rearrangement problems concentrates on building a \emph{region graph} of the objects by decomposing the space and applying a depth-first search. Our method differs from the idea of extracting the minimal number of actions from possible permutations to solve the problem. Instead, we plan efficiently based on our factored state-space and interpolation method and optimize the solution path afterward.  










%Our approach relies on finding optimal solutions to motion planning problems in a factored state space. This is closely related to planners like the Manhattan-like RRT~\cite{Cortes2007}, where planning is decomposed into an active and a passive subspace. Planning is done exclusively in the active subspace, while the passive subspace is only sampled when obstructions are detected (for example, when a door blocks an object). Our planner generalizes this idea, makes it applicable to manipulation, and combines it with optimality, such that we find the minimal amount of switches between subspaces.

%Furthermore, our approach aims to minimize the necessary number of actions to solve the problem. It has also been explored in assembly sequence planning approaches~\cite{masehian2020asppr}, where the goal is to find an action sequence with the minimum number of \emph{relocations} by focusing on the interferences between the objects. Our method differs from the idea of extracting the minimal number of actions from all possible permutations to solve the assembly problem. Instead, we plan efficiently based on our factored state-space and interpolation method and optimize the solution path afterward.  

%Recently, new planners have been developed, which solve difficult mechanical puzzles~\cite{zhang2020cspace}. Such planner rely on machine learning to identify narrow passages in the environment, which can then be sampled with a higher probability. This approach, however, only works for rigid bodies, while our approach can be applied to any articulated puzzle, without restrictions on the degrees-of-freedom. We also explicitly integrate a robot, which should eventually solve such puzzles.


% \section{Related Work}

% We first discuss the classical approaches to solve logic-geometric puzzles. Afterwards, we discuss methods which are closely related to motion planning in our factored state space. 

% \subsection{Frameworks to Solve Logic-Geometric Puzzles}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% First, we can solve logic-geometric puzzles using a \emph{symbolic planning approach}~\cite{toussaint2018RSS, Hartmann2021TRO}. In such an approach, we create a search graph over symbolic actions (e.g. pick, place), applicable to each of the objects in the scene. A valid path through this search graph provides an action skeleton, a set of constraints which we can use for motion planning~\cite{Grothe2022} or differentiable optimizer~\cite{toussaint2015IJCAI}. If an action skeleton is infeasible, expensive backtracking has to be performed~\cite{20-driess-RSS} to validate another action skeleton. In scenes with multiple objects, which have to be moved out of the way to solve the problem, such approaches spend considerable time re-validating action skeletons. 

% Our work is complementary, in that we also use pick-place symbols for our robot, but we choose those symbols \emph{implicitly} using the (admissible) heuristic from our \puzzlealgo planner, which gives us a complete valid sequential solution path for all objects involved. This tighter integration of planning and robot capabilties give us a better chance to avoid expensive backtracking.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Second, we can solve logic-geometric puzzles using a \emph{constrained-based planning approach}~\cite{kingston2018sampling, Kingston2019, vega2020asymptotically}. Instead of relying on symbols, in this approach, we enumerate all constraints using a constraint graph~\cite{mirabel2017manipulation}, which provides information about the inter-connectivity of constraint sets. To find solutions, we can employ constrained-based sampling, where uniform sampling is combined with projection methods, which project samples down onto a desired constraint-set or used as steering method~\cite{berenson2011task, Kingston2019}. Such method avoid the difficulty of finding good symbols for a particular problem, but they become sample-inefficient, when the projection methods do not adequately cover all constraint-sets. 

% Our approach differs, in that we do not plan directly in the full robot-object configuration space, which would be too costly to execute. Instead, we integrate the capabilities of the robot into the motion planner using the new factored state space to ensure that the correct paths are returned.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Motion planning for Logic-Geometric Puzzles}

% Our approach relies on finding optimal solutions to motion planning problems in a factored state space. This is closely related to planners like the Manhattan-like RRT~\cite{Cortes2007}, where planning is decomposed into an active and a passive subspace. Planning is done exclusively in the active subspace, while the passive subspace is only sampled when obstructions are detected (for example, when a door blocks an object). Our planner generalizes this idea, makes it applicable to manipulation, and combines it with optimality, such that we find the minimal amount of switches between subspaces.

% %Recently, new planners have been developed, which solve difficult mechanical puzzles~\cite{zhang2020cspace}. Such planner rely on machine learning to identify narrow passages in the environment, which can then be sampled with a higher probability. This approach, however, only works for rigid bodies, while our approach can be applied to any articulated puzzle, without restrictions on the degrees-of-freedom. We also explicitly integrate a robot, which should eventually solve such puzzles.

==> src/algorithms/manipulate.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$solutionPath$}

$Actions \longleftarrow$ \textsc{extractActions}($solutionPath$)\;
\ForEach{$action$ in $Actions$}{
    $obj \longleftarrow \textsc{GetObject}(action$)\;
    
    \While{true}{
     \lIf{Not \textsc{graspObject}(obj)}{
        \textsc{Continue}
     }
     $cstr \longleftarrow \textsc{GetCSTR}(obj.link,robot.wrist\_link)$\;
     
     \lIf{\textsc{tryAction}($obj,action, cstr$)}{
        \textsc{Break}
     }
    }
    }

\caption{\textsc{ManipulateWithRobot}\label{alg:manipulate}}
\end{algorithm}



==> src/algorithms/tryskipfragment.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwIn{$P$}

\SetKwRepeat{Do}{do}{while}
\Do{ $\textsc{Cost}(P) < cost_{old} $ }
{

    $cost_{old} \longleftarrow$ \textsc{Cost}$(P)$ \;
    
    $F \longleftarrow \textsc{getFragmentIntervals}(P)$ 

\For{i=1  \KwTo  $F.size$}{
    
        $P_{a} \longleftarrow \textsc{getStates}(1,F[i]_{start}, P)$\;
        $P_{b} \longleftarrow \textsc{getStates}(F[i]_{end}+1, P.size, P)$\;
        
        $P_{result} \longleftarrow \textsc{ReConnect} (P_{a},P_{b}$)\;
    
    \If{!$P_{result}$.empty}{
            
            $P = P_{result}$\;
            $F = \textsc{getFragmentIDs}(P)$\;
        }
}

}

\caption{\textsc{TrySkipFragment}\label{alg:tryskipfragment}}
\end{algorithm}
